Architecture Diagrams: A Graphical Language for Architecture Style Specification

Architecture styles characterise families of architectures sharing common characteristics. We have recently proposed configuration logics for architecture style specification. In this paper, we study a graphical notation to enhance readability and easiness of expression. We study simple architecture diagrams and a more expressive extension, interval architecture diagrams. For each type of diagrams, we present its semantics, a set of necessary and sufficient consistency conditions and a method that allows to characterise compositionally the specified architectures. We provide several examples illustrating the application of the results. We also present a polynomial-time algorithm for checking that a given architecture conforms to the architecture style specified by a diagram.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{M. Bartoletti, L. Henrio, S. Knight, and H. T. Vieira (Eds.):\\9th Interaction and Concurrency Experience (ICE 2016)\\
EPTCS 223, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.223.6}{10.4204/EPTCS.223.6}}
\pdfoutput=1

